Node Classification With Integrated Reject Option

One of the key tasks in graph learning is node classification. While Graph neural networks have been used for various applications, their adaptivity to reject option setting is not previously explored. In this paper, we propose NCwR, a novel approach to node classification in Graph Neural Networks (GNNs) with an integrated reject option, which allows the model to abstain from making predictions when uncertainty is high. We propose both cost-based and coverage-based methods for classification with abstention in node classification setting using GNNs. We perform experiments using our method on three standard citation network datasets Cora, Citeseer and Pubmed and compare with relevant baselines. We also model the Legal judgment prediction problem on ILDC dataset as a node classification problem where nodes represent legal cases and edges represent citations. We further interpret the model by analyzing the cases that the model abstains from predicting by visualizing which part of the input features influenced this decision.

==> Images/ildc.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{Images/comparision/ildc.png}
    \caption{Comparison of NCwR-Cost and NCwR-Cov in ILDC Dataset.}
    \label{fig:ildc}
\end{figure}

==> Tables/baseline.tex <==
% \begin{table}[]
%     \centering
%     \raa{1.2}
%     \begin{tabular}{@{}rrrr@{}}\toprule
%     SR & CF-GNN & NCwR-Cov & NCwR-Cost\\ \midrule
%     & $91.00$ {\scriptsize ($65.70$)} & $93.96$ {\scriptsize ($50$)} & $95.8$ {\scriptsize ($42.6$)}\\
%     & $88.00$ {\scriptsize ($72.53$)} & $92.65$ {\scriptsize ($60$)} & $95.0$ {\scriptsize ($53.1$)}\\
%     & $86.49$ {\scriptsize ($76.58$)} & $91.29$ {\scriptsize ($70$)} & $92.8$ {\scriptsize ($66.3$)}\\
%     & $85.66$ {\scriptsize ($79.14$)} & $89.12$ {\scriptsize ($80$)} & $90.1$ {\scriptsize ($83.3$)}\\
%     & $79.93$ {\scriptsize ($87.02$)} & $86.65$ {\scriptsize ($90$)} & $87.2$ {\scriptsize ($90.5$)}\\
%     \bottomrule
%     \end{tabular}
%     \caption{Comparison of our method with various baselines. The results are presented in the format Accuracy {\scriptsize (Coverage)}}
%     \label{tab:baseline}
% \end{table}


==> Tables/ildc_cwr.tex <==
% \begin{table*}\centering
% \raa{1.7}
% \begin{tabular}{@{}ccc@{}}\toprule
% % \multicolumn{3}{c}{ILDC}\\
% % \cmidrule{1-3}
% $d$ & Acc & Cov \\ \midrule

% $0.25$ & 
% % $\substack{\text{\normalsize 95.8} \\ \text{\scriptsize $\pm$ 0.05}}$ & $\substack{\text{\normalsize 42.6} \\ \text{\scriptsize $\pm$ 0.05}}$ \\
% \multicolumn{1}{c}{$87.23\pm2.45$} & \multicolumn{1}{c}{$67.00\pm3.30$} \\
% $0.35$ & 
% \multicolumn{1}{c}{$82.32\pm2.72$} & \multicolumn{1}{c}{$86.34\pm4.61$} \\
% $0.40$ & 
% \multicolumn{1}{c}{$79.95\pm1.52$} & \multicolumn{1}{c}{$93.44\pm7.17$} \\
% $0.45$ & 
% \multicolumn{1}{c}{$80.38\pm1.74$} & \multicolumn{1}{c}{$97.83\pm0.76$} \\
% $0.50$ & 
% \multicolumn{1}{c}{$79.94\pm2.09$} & \multicolumn{1}{c}{$98.99\pm0.20$} \\
% \bottomrule
% \end{tabular}
% \caption{Accuracy of NCwR-Cost for various cost of rejection values on ILDC.}
% \label{tab:ildc_cost}
% \end{table*}

==> Tables/ildc_sn.tex <==
% \begin{table*}
% \centering
% \raa{1.2}

% \begin{tabular}{rr||cc}\toprule
% & \multicolumn{1}{c}{Coverage} & \multicolumn{1}{c}{Acc} &  \\
% \bottomrule
% &\multicolumn{1}{c}{$0.5$} & \multicolumn{1}{c}{$97.55\pm0.62$} & \\
% &\multicolumn{1}{c}{$0.6$} & \multicolumn{1}{c}{$94.94\pm1.20$} & \\
% &\multicolumn{1}{c}{$0.7$} & \multicolumn{1}{c}{$90.58\pm1.24$} & \\
% &\multicolumn{1}{c}{$0.8$} & \multicolumn{1}{c}{$86.01\pm1.09$} & \\
% &\multicolumn{1}{c}{$0.9$} & \multicolumn{1}{c}{$81.87\pm1.03$} & \\
% \bottomrule
% \end{tabular}
% \caption{Accuracy of NCwR-Cov for various coverage rates on ILDC.}
% \label{tab:ildc_sn}
% \end{table*}

==> Tables/thyroid.tex <==
\begin{table*}\centering
\raa{1.1}
\begin{tabular}{@{}cccp{0.1cm}cc@{}} \toprule
\multicolumn{3}{c}{NCwR-Cost} & \phantom{abc} & \multicolumn{2}{c}{NCwR-Cov}\\
\cmidrule{1-3} \cmidrule{5-6} 
$d$ & Acc & Cov && Cov & Acc \\ \midrule
$0.05$ & {$96.56\pm0.68$} & {$60.52\pm9.21$} &&{$0.5$} & {$99.66\pm0.09$} \\
$0.10$ & {$96.40\pm0.13$} & {$82.37\pm2.39$} &&{$0.6$} & {$99.53\pm0.06$} \\
$0.20$ & {$95.29\pm0.40$} & {$94.09\pm0.84$} &&{$0.7$} & {$99.31\pm0.10$} \\
$0.30$ & {$94.37\pm0.21$} & {$98.20\pm0.18$} &&{$0.8$} & {$98.75\pm0.09$} \\
$0.40$ & {$93.75\pm0.18$} & {$99.76\pm0.13$} &&{$0.9$} & {$97.48\pm0.04$} \\
\bottomrule
\end{tabular}
\caption{Accuracy of NCwR-Cost and NCwR-Cov for various cost of rejection values and coverage rates respectively on Thyroid dataset.}
\label{tab:cost_cov_thy}
\end{table*}
